Classification of Spam URLs Using Machine Learning Approaches

The Internet is used by billions of users every day because it offers fast and free communication tools and platforms. Nevertheless, with this significant increase in usage, huge amounts of spam are generated every second, which wastes internet resources and, more importantly, users' time. This study investigates the use of machine learning models to classify URLs as spam or nonspam. We first extract the features from the URL as it has only one feature, and then we compare the performance of several models, including k nearest neighbors, bagging, random forest, logistic regression, and others. Experimental results demonstrate that bagging outperformed other models and achieved the highest accuracy of 98.64%. In addition, bagging outperformed the current state-of-the-art approaches which emphasize its effectiveness in addressing spam-related challenges on the Internet. This suggests that bagging is a promising approach for URL spam classification.

==> results.tex <==

In this section of the paper, we will show and discuss the results for each model. This includes showing the tuned hyperparameters, confusion matrix, ROC, AUC, and finally the model scores.

\subsection{Logistic regression}
The logistic regression model was implemented using the following tuned hyperparameters:
\begin{table}[!htbp]
\caption{Logistic regression hyperparameters}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{FCFF2F} 
Parameter                 & Value     \\ \hline
\cellcolor[HTML]{FFFFFF}
C                         & 100       \\ \hline
class\_weight             & None      \\ \hline
dual                      & False     \\ \hline
fit\_intercept            & True      \\ \hline
intercept\_scaling        & 1         \\ \hline
l1\_ratio                 & None      \\ \hline
max\_iter                 & 140       \\ \hline
multi\_class              & auto      \\ \hline
n\_jobs                   & None      \\ \hline
penalty                   & l2        \\ \hline
random\_state             & None      \\ \hline
solver                    & liblinear \\ \hline
tol                       & 0.0001    \\ \hline
verbose                   & 0         \\ \hline
warm\_start               & False     \\ \hline
\end{tabular}
\end{table}

\newpage
The next figure shows the ROC and AUC charts, this model has a good AUC value equal to 0.87.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.35]{results/lr-roc.png}
  \caption{Logistic regression ROC and AUC}
\end{figure}

Finally, below are the scores of the model. This model shows relatively poor results with a k-fold accuracy equal to ~82\% and a small R square far away from 1.
\begin{table}[!htbp]
\caption{Logistic regression scores}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\cellcolor[HTML]{F8FF00}Metric & \cellcolor[HTML]{F8FF00}Result \\ \hline
Accuracy                       & 82.19\%                        \\ \hline
Precision                      & 74.42\%                        \\ \hline
Recall                         & 66.75\%                        \\ \hline
R square                       & 0.18                           \\ \hline
F1 score                       & 70.38\%                        \\ \hline
Kfold(k=5) accuracy                 & 82.22\%                        \\ \hline
\end{tabular}
\end{table}

\subsection{Multi layer perceptron (MLP)}
The MPL - Neural network model was tested using the following tuned hyperparameters as in the next table.
\begin{table}[!htbp]
\caption{MLP hyperparameters}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{FCFF2F} 
Parameter                 & Value     \\ \hline
\cellcolor[HTML]{FFFFFF}C & 100       \\ \hline
alpha                              & 0.1                           \\ \hline
batch\_size                        & auto                          \\ \hline
beta\_1                            & 0.9                           \\ \hline
epsilon                            & 1e-08                         \\ \hline
hidden\_layer\_sizes               & (14, 9)                       \\ \hline
learning\_rate                     & adaptive                      \\ \hline
learning\_rate\_init               & 0.001                         \\ \hline
max\_fun                           & 15000                         \\ \hline
max\_iter                          & 240                           \\ \hline
momentum                           & 0.9                           \\ \hline
n\_iter\_no\_change                & 10                            \\ \hline
power\_t                           & 0.5                           \\ \hline
random\_state                      & None                          \\ \hline
shuffle                            & True                          \\ \hline
solver                             & adam                          \\ \hline
tol                                & 0.0001                        \\ \hline
validation\_fraction               & 0.1                           \\ \hline
\end{tabular}
\end{table}

Below is the confusion matrix, which shows a lower number of false positives and false negatives in the prediction compared to the logistic regression model.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.35]{results/mlp-conf.png}
  \caption{MLP confusion matrix}
\end{figure}


The next figure shows the ROC and AUC charts, this model has a very good AUC value equals 0.92.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.45]{results/mlp-roc.png}
  \caption{Multi layer perceptron ROC and AUC}
\end{figure}

Finally, below are the scores of the model:
\begin{table}[!htbp]
\caption{Multi layer perceptron scores}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\cellcolor[HTML]{F8FF00}Metric & \cellcolor[HTML]{F8FF00}Result \\ \hline
Accuracy                       & 85.33\%                        \\ \hline
Precision                      & 76.52\%                        \\ \hline
Recall                         & 77.49\%                        \\ \hline
R square                       & 0.32                           \\ \hline
F1 score                       & 77\%                           \\ \hline
Kfold(k=5) accuracy                 & 84.26\%                        \\ \hline
\end{tabular}
\end{table}

This model shows a better accuracy and a better r2 compared to the previous trained model, but 84.26\% it's still not reliable for spam detection.

\subsection{KNeighbours classifier}
The KNeighbours model gave it's best results with the following tuned hyperparameters:
\begin{table}[!htbp]
\caption{KNeighbours hyperparameters}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{FCFF2F} 
Parameter                 & Value     \\ \hline
\cellcolor[HTML]{FFFFFF}C & 100       \\ \hline
algorithm      & auto                          \\ \hline
leaf\_size     & 30                            \\ \hline
metric         & minkowski                     \\ \hline
metric\_params & None                          \\ \hline
n\_jobs        & None                          \\ \hline
n\_neighbors   & 1                             \\ \hline
p              & 2                             \\ \hline
weights        & uniform                       \\ \hline
\end{tabular}
\end{table}

Below is the confusion matrix, which shows a great results with few number of both false positives and negatives. So far, it shows the best confusion matrix.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.35]{results/k-conf.png}
  \caption{KNeighbours confusion matrix}
\end{figure}


The next figure shows the ROC and AUC charts, this model has an excellent AUC value equals 0.95.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.45]{results/k-roc.png}
  \caption{KNeighbours ROC and AUC}
\end{figure}
\newline

Finally, below table presents the scores of the model. The model shows great accuracy and a good r2 that is close to 1. Finally, we've crossed the 90 percent mark with +93.3\% accuracy.
\newline
\begin{table}[!htbp]
\caption{KNeighbours  scores}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\cellcolor[HTML]{F8FF00}Metric & \cellcolor[HTML]{F8FF00}Result \\ \hline
Accuracy                       & 95.09\%                        \\ \hline
Precision                      & 91.16\%                        \\ \hline
Recall                         & 93.59\%                        \\ \hline
R square                       & 0.77                           \\ \hline
F1 score                       & 92.36\%                           \\ \hline
Kfold(k=5) accuracy            & 93.34\%                        \\ \hline
\end{tabular}
\end{table}



\subsection{Gradient Boosting classifier}
The Gradient Boosting model was used with the following tuned hyperparameters:
\begin{table}[!htbp]
\caption{Gradient Boosting hyperparameters}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{FCFF2F} 
Parameter                 & Value     \\ \hline
\cellcolor[HTML]{FFFFFF}C & 100       \\ \hline
ccp\_alpha                  & 0.0                           \\ \hline
criterion                   & friedman\_mse                 \\ \hline
init                        & None                          \\ \hline
learning\_rate              & 0.3                           \\ \hline
loss                        & deviance                      \\ \hline
max\_depth                  & 9                             \\ \hline
min\_impurity\_decrease     & 0.0                           \\ \hline
min\_samples\_leaf          & 1                             \\ \hline
min\_samples\_split         & 2                             \\ \hline
min\_weight\_fraction\_leaf & 0.0                           \\ \hline
n\_estimators               & 110                           \\ \hline
subsample                   & 1                             \\ \hline
tol                         & 0.0001                        \\ \hline
validation\_fraction        & 0.1                           \\ \hline
\end{tabular}
\end{table}

Below is the confusion matrix, which shows the best results so far with a few number of both false positives and negatives.

\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.35]{results/gbc-ocnf.png}
  \caption{Gradient Boosting confusion matrix}
\end{figure}


The next figure shows the ROC and AUC charts, this model has an outstanding AUC value equals 0.99.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.45]{results/gbc-roc.png}
  \caption{Gradient Boosting ROC and AUC}
\end{figure}
\newpage
Finally, below are the scores of the model. This model shows the best k-fold accuracy = 94.54\% comparing to the previous models and a very good r2 that is very close to 1. It also shows a very high score of all other metrics such as precision, recall, and F1 score. All measures are +90\%.
\begin{table}[!htbp]
\caption{Gradient Boosting scores}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\cellcolor[HTML]{F8FF00}Metric & \cellcolor[HTML]{F8FF00}Result \\ \hline
Accuracy                       & 95.90\%                        \\ \hline
Precision                      & 92.73\%                      \\ \hline
Recall                         & 94.46\%                        \\ \hline
R square                       & 0.81                           \\ \hline
F1 score                       & 93.59\%                           \\ \hline
Kfold(k=5) accuracy                 & 94.54\%                        \\ \hline
\end{tabular}
\end{table}

\subsection{Decision Tree classifier}
The Decision Tree model gave it's best results with the following tuned hyperparameters:
\begin{table}[!htbp]
\caption{Decision Tree hyperparameters}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{FCFF2F} 
Parameter                 & Value     \\ \hline
\cellcolor[HTML]{FFFFFF}C & 100       \\ \hline
ccp\_alpha                  & 0.0                           \\ \hline
class\_weight               & None                          \\ \hline
criterion                   & entropy                       \\ \hline
max\_depth                  & 22                            \\ \hline
max\_features               & None                          \\ \hline
max\_leaf\_nodes            & None                          \\ \hline
min\_impurity\_decrease     & 0.0                           \\ \hline
min\_samples\_leaf          & 1                             \\ \hline
min\_samples\_split         & 2                             \\ \hline
min\_weight\_fraction\_leaf & 0.0                           \\ \hline
random\_state               & None                          \\ \hline
splitter                    & best                          \\ \hline
\end{tabular}
\end{table}

Below is the confusion matrix, which shows superior results compared to the first 2 models (MLP and Logistic regression), but it has more falsy values than the last 2 models.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.35]{results/dtc-conf.png}
  \caption{Decision Tree confusion matrix}
\end{figure}
\newpage
The next figure shows the ROC and AUC charts, this model has an excellent AUC value equals 0.98.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.45]{results/dtc-roc.png}
  \caption{Decision Tree ROC and AUC}
\end{figure}

Finally, below are the scores of the model. This model shows a very good measure with a k fold accuracy = 92.42\% and a very good r2 of 1. This is the third best model after k neighbors and gradient boosting.
\begin{table}[!htbp]
\caption{Decision Tree scores}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\cellcolor[HTML]{F8FF00}Metric & \cellcolor[HTML]{F8FF00}Result \\ \hline
Accuracy                       & 93.66\%                        \\ \hline
Precision                      & 90.37\%                      \\ \hline
Recall                         & 89.56\%                        \\ \hline
R square                       & 0.71                         \\ \hline
F1 score                       & 89.96\%                           \\ \hline
Kfold(k=5) accuracy                 & 92.42\%                        \\ \hline
\end{tabular}
\end{table}

\subsection{Naive Bayes - Bernoulli}
The Naive Bayes model gave it's best results with the following tuned hyperparameters:
\begin{table}[!htbp]
\caption{Naive Bayes hyperparameters}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{FCFF2F} 
Parameter                 & Value     \\ \hline
\cellcolor[HTML]{FFFFFF}C & 100       \\ \hline
alpha                  & 10           \\ \hline
binarize               & 0            \\ \hline
class\_prior            & None         \\ \hline
fit\_prior              & True         \\ \hline
\end{tabular}
\end{table}

Below is the confusion matrix, which shows a very high number of false negatives. Overall, it shows the worst predictions so far.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.35]{results/nbc-conf.png}
  \caption{Naive Bayes confusion matrix}
\end{figure}

The next figure shows the ROC and AUC charts, This model has a poor AUC value equals 0.8 compared to the previous models.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.40]{results/nbc-roc.png}
  \caption{Naive Bayes ROC and AUC}
\end{figure}
\newpage
Finally, below are the scores of the model. This model shows the worst results so far. It has a negative R2 and an accuracy below 78\% which can be considered as a bad model, especially for a binary classification.
\begin{table}[!htbp]
\caption{Naive Bayes scores}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\cellcolor[HTML]{F8FF00}Metric & \cellcolor[HTML]{F8FF00}Result \\ \hline
Accuracy                       & 78.17\%                        \\ \hline
Precision                      & 84.62\%                      \\ \hline
Recall                         & 38.03\%                        \\ \hline
R square                       & -0.01                         \\ \hline
F1 score                       & 52.48\%                           \\ \hline
Kfold(k=5) accuracy                 & 78.15\%                        \\ \hline
\end{tabular}
\end{table}

\subsection{Ada Boost Classifier}
The Ada Boost model gave it's best results with the following tuned hyperparameters:
\begin{table}[!htbp]
\caption{Ada Boost hyperparameters}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{FCFF2F} 
Parameter                 & Value     \\ \hline
\cellcolor[HTML]{FFFFFF}C & 100       \\ \hline
algorithm       & SAMME.R                       \\ \hline
base\_estimator & None                          \\ \hline
learning\_rate  & 1.5                           \\ \hline
n\_estimators   & 90                            \\ \hline
random\_state   & None                          \\ \hline
\end{tabular}
\end{table}

Below is the confusion matrix, which shows a high number of both false positives and negatives. It's one of the three worst confusion matrices.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.35]{results/ada-conf.png}
  \caption{Ada Boost confusion matrix}
\end{figure}


The next figure shows the ROC and AUC charts, this model has a good AUC value equals 0.91.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.45]{results/ada-roc.png}
  \caption{Ada Boost ROC and AUC}
\end{figure}
\newline
Finally, below are the scores of the model:
\begin{table}[!htbp]
\caption{Ada Boost scores}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\cellcolor[HTML]{F8FF00}Metric & \cellcolor[HTML]{F8FF00}Result \\ \hline
Accuracy                       & 84.22\%                        \\ \hline
Precision                      & 77.21\%                      \\ \hline
Recall                         & 71.23\%                        \\ \hline
R square                       & 0.27                         \\ \hline
F1 score                       & 74.10\%                           \\ \hline
Kfold(k=5) accuracy                 & 84.30\%                        \\ \hline
\end{tabular}
\end{table}

This model shows a very close score to MLP classifier. The accuracy isn't reliable in this model for spam detection.

\subsection{Random Forest Classifier}
The Random Forest model gave it's best results comparing to the previous models with the following tuned hyperparameters:
\begin{table}[!htbp]
\caption{Random Forest hyperparameters}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{FCFF2F} 
Parameter                 & Value     \\ \hline
\cellcolor[HTML]{FFFFFF}C & 100       \\ \hline
bootstrap                   & True                          \\ \hline
ccp\_alpha                  & 0.0                           \\ \hline
class\_weight               & None                          \\ \hline
criterion                   & gini                          \\ \hline
max\_depth                  & 23                            \\ \hline
max\_features               & None                          \\ \hline
max\_leaf\_nodes            & None                          \\ \hline
max\_samples                & None                          \\ \hline
min\_impurity\_decrease     & 0.0                           \\ \hline
min\_samples\_leaf          & 1                             \\ \hline
min\_samples\_split         & 2                             \\ \hline
min\_weight\_fraction\_leaf & 0.0                           \\ \hline
n\_estimators               & 20                            \\ \hline
n\_jobs                     & None                          \\ \hline
oob\_score                  & False                         \\ \hline
random\_state               & None                          \\ \hline
verbose                     & 0                             \\ \hline
warm\_start                 & False                         \\ \hline
\end{tabular}
\end{table}

Below  is  the confusion matrix,  which shows the best results so far. In fact, it shows the least number of false negatives compared to all other models.\newline
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.35]{results/rf-conf.png}
  \caption{Random Forest confusion matrix}
\end{figure}


The next figure shows the  ROC  and  AUC charts, This model has an outstanding AUC value equals 0.99 similar to gradient boosting results.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.45]{results/rf-roc.png}
  \caption{Random Forest ROC and AUC}
\end{figure}

Finally, below are the scores of the model:
\begin{table}[!htbp]
\caption{Random Forest scores}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\cellcolor[HTML]{F8FF00}Metric & \cellcolor[HTML]{F8FF00}Result \\ \hline
Accuracy                       & 95.94\%                        \\ \hline
Precision                      & 92.68\%                      \\ \hline
Recall                         & 94.65\%                        \\ \hline
R square                       & 0.81                         \\ \hline
F1 score                       & 93.66\%                           \\ \hline
Kfold(k=5) accuracy                 & 94.64\%                        \\ \hline
\end{tabular}
\end{table}

The random forest model shows better results compared to all previous models. However, It showed very close and almost identical results to gradient boosting scores with an accuracy equals 94.64\%.
\subsection{Bagging Classifier}
The Bagging Classifier gave it's best results with the following tuned hyperparameters:
\begin{table}[!htbp]
\caption{Bagging hyperparameters}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{F8FF00} 
Parameter           & \cellcolor[HTML]{F8FF00}Value \\ \hline
base\_estimator     & None                          \\ \hline
bootstrap           & True                          \\ \hline
bootstrap\_features & False                         \\ \hline
max\_features       & 1.0                           \\ \hline
max\_samples        & 1.0                           \\ \hline
n\_estimators       & 140                           \\ \hline
n\_jobs             & None                          \\ \hline
oob\_score          & False                         \\ \hline
random\_state       & None                          \\ \hline
verbose             & 0                             \\ \hline
warm\_start         & False                         \\ \hline
\end{tabular}
\end{table}

Below is the confusion matrix, which shows a great results, and it has the lowest false negatives compared to all other models.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.65]{results/1212.png}
  \caption{Bagging confusion matrix}
\end{figure}
\newpage
The next figure shows the ROC and AUC charts, this model has an excellent AUC value equals 0.994.
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.8]{results/10.png}
  \caption{Bagging ROC and AUC}
\end{figure}
\newline
Finally, below are the scores of the model:\newline
\begin{table}[!htbp]
\caption{Bagging scores}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\cellcolor[HTML]{F8FF00}Metric & \cellcolor[HTML]{F8FF00}Result \\ \hline
Accuracy                       & 96.52\%                        \\ \hline
Precision                      & 93.26\%                      \\ \hline
Recall                         & 95.98\%                        \\ \hline
R square                       & 0.84                         \\ \hline
F1 score                       & 94.60\%                           \\ \hline
Kfold(k=5) accuracy                 & 95.10\%                        \\ \hline
\end{tabular}
\end{table}

This model shows the best k fold accuracy = 95.10\% and a the best r2 of 0.84. This is the best model so far.
\subsection{Stacking Classifier}
The Stacking Classifier gave it's best results with the following tuned hyperparameters:
\begin{table}[!htbp]
\caption{Stacking hyperparameters}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|l|}
\hline
\rowcolor[HTML]{F8FF00} 
Parameter        & \cellcolor[HTML]{F8FF00}Value \\ \hline
final\_estimator & None                          \\ \hline
n\_jobs          & None                          \\ \hline
passthrough      & False                         \\ \hline
stack\_method    & auto                          \\ \hline
verbose          & 0                             \\ \hline
BC               & BaggingClassifier             \\ \hline
RFC              & RandomForestClassifier        \\ \hline
DT               & DecisionTreeClassifier        \\ \hline
GBC              & GradientBoostingClassifier    \\ \hline
\end{tabular}
\end{table}
\newpage
Below is the confusion matrix, which shows very good results compared to most models, but it has more falsy values than the Bagging classifier.

\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.65]{results/13.png}
  \caption{Stacking confusion matrix}
\end{figure}
The next figure shows the ROC and AUC charts, this model has an excellent AUC value equal to 0.994.
\newline
\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.85]{results/1414.PNG}
  \caption{Stacking ROC and AUC}
\end{figure}

Finally, below are the scores of the model. This model shows a very good measure with a k-fold accuracy = 94.82\% and a very good r2 of 0.82. This is the second-best model after the Bagging Classifier.
\begin{table}[!htbp]
\caption{Stacking scores}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{|l|
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\cellcolor[HTML]{F8FF00}Metric & \cellcolor[HTML]{F8FF00}Result \\ \hline
Accuracy                       & 96.21\%                        \\ \hline
Precision                      & 94.53\%                      \\ \hline
Recall                         & 93.44\%                        \\ \hline
R square                       & 0.82                         \\ \hline
F1 score                       & 93.98\%                           \\ \hline
Kfold(k=5) accuracy                 & 94.82\%                        \\ \hline
\end{tabular}
\end{table}

\newpage
\section{Models comparison}

Stacking and bagging classifier show the best precision, recall and f1 scores. On the other hand, both naive bayes models have the worst measures. 

\begin{table}[!htbp]
\caption{Comparison results of Precision, Recall, and F1 score}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{llll}
\hline
Classifier                  & Precision & Recall  & F1 score \\ \hline
Logistic regression         & 74.42\%   & 66.75\% & 70.38\%  \\
KNeighbours                 & 91.16\%   & 93.59\% & 92.36\%  \\
Ada Boost                   & 77.21\%   & 71.23\% & 74.10\%  \\
Multinominal & 54.06\%   & 83.07\% & 65.50\%  \\
Bernoulli    & 84.62\%   & 38.03\% & 52.48\%  \\
Random forest               & 92.68\%   & 94.65\% & 93.66\%  \\
Gradient boosting           & 92.73\%   & 94.46\% & 93.59\%  \\
Multilayer perceptron       & 76.52\%   & 77.49\% & 77.00\%  \\
Bagging              & 93.26\%  & 95.98     & 94.60\%        \\
Stacking             & 94.53\%  & 93.44     & 93.98\%        \\
Decision tree               & 90.37\%   & 89.56\% & 89.96\% 
\end{tabular}
\end{table}

\begin{table}[!htbp]
\caption{Comparison results of Accuracy, R square, and K-fold}
\small
\centering
\captionsetup{justification=centering}
\begin{tabular}{llll}
\hline
Classifier                  & Accuracy & R square & K-fold \\ \hline
Logistic regression         & 82.19\%  & 0.18     & 82.22\%        \\
KNeighbours                 & 95.09\%  & 0.77     & 93.34\%        \\
Ada Boost                   & 84.22\%  & 0.27     & 84.30\%        \\
Multinominal & 72.26\%  & -0.28    & 72.41\%        \\
Bernoulli    & 78.17\%  & -0.01    & 78.15\%        \\
Random forest               & 95.94\%  & 0.81     & 94.64\%        \\
Gradient boosting           & 95.90\%  & 0.81     & 94.54\%        \\
Multilayer perceptron       & 85.33\%  & 0.32     & 84.26\%        \\
Bagging           & 96.52\%  & 0.84     & 95.10\%        \\
Stacking       & 96.21\%  & 0.82     & 94.82\%        \\
Decision tree               & 93.66\%  & 0.71     & 92.42\%       
\end{tabular}
\end{table}

\begin{enumerate}
  \item The top three models with the highest accuracy are Bagging with accuracy equals 96.52\% and kfold accuracy 95.1 \%, then Stacking classifier with accuracy equals 96.21\% and kfold accuracy 94.82 \%, and finally Random forest with accuracy equals 95.94\% and kfold accuracy 94.64 \%.
  \newline
  \item Both naive bayes models showed the worst accuracy numbers, they are the only models that had an accuracy less than 80\% - 72\% for the multinominal and 78\% for the bernoulli.
  \newline
  \item There are four models with an R square more than 0.8 which are the bagging with r2 = 0.84, stacking with r2 = 0.82 and finally random forest and gradient boosting. Both models had an R square equals 0.81.
  \newline
  \item Bagging classifier showed the best results among all metrics, with results around 95\% in precision, recall, accuracy and F1 score.
\end{enumerate}

\begin{figure}[ht]
\centering
\captionsetup{justification=centering}
  \includegraphics[scale=0.660]{results/ttt.PNG}
  \caption{Models comparison ROC and AUC}
\end{figure}

The previous chart shows a full comparison of ROC curves and AUC values between all different models that have been experimented with and trained for the spam URL dataset. As discussed previously, It shows that the bagging and stacking models have the best true positive rates with the best AUC values equaling 0.994. It also shows the worst models which are both naive bayes models (Multinominal and Bernouli).  
